Empirical determination of the shape of dust attenuation curves in star-forming galaxies

We present a systematic study of the shape of the dust attenuation curve in star-forming galaxies from the far ultraviolet to the near infrared (0.15-2microns), as a function of specific star formation rate (sSFR) and axis ratio (b/a), for galaxies with and without a significant bulge. Our sample comprises 23,000 (15,000) galaxies with a median redshift of 0.07, with photometric entries in the SDSS, UKIDSS-LAS (and GALEX-AIS) survey catalogues and emission line measurements from the SDSS spectroscopic survey. We develop a new pair-matching technique to isolate the dust attenuation curves from the stellar continuum emission. The main results are: (i) the slope of the attenuation curve in the optical varies weakly with sSFR, strongly with b/a, and is significantly steeper than the Milky Way extinction law in bulge-dominated galaxies; (ii) the NIR slope is constant, and matches the slope of the Milky Way extinction law; (iii) the UV has a slope change consistent with a dust bump at 2175AA which is evident in all samples and varies strongly in strength with b/a in the bulge-dominated sample; (iv) there is a strong increase in emission line-to-continuum dust attenuation with both decreasing sSFR and increasing b/a; (v) radial gradients in dust attenuation increase strongly with increasing sSFR, and the presence of a bulge does not alter the strength of the gradients. These results are consistent with the picture in which young stars are surrounded by dense `birth clouds' with low covering factor which disperse on timescales of ~1e7 years and the diffuse interstellar dust is distributed in a centrally concentrated disk with a smaller scaleheight than the older stars that contribute the majority of the red and NIR light. [abridged]

==> code.tex <==
\begin{code*}
{\bf /* To obtain parameters for spectroscopic galaxies in the SDSS */}
\begin{verbatim}
/* Basic parameters */
SELECT  s.bestobjid,s.specobjid, mjd,plate,fiberid,s.z,sn_0,sn_1,
petror50_r,petror90_r,petror50_z,rowindex, p.extinction_g, p.petrorad_r,

/* Petrosian magnitudes */
p.petromag_u, p.petromag_g, p.petromag_r, p.petromag_i, p.petromag_z,

/* The number of annuli for which there is a measurable signal */
p.nprof_u, p.nprof_g, p.nprof_r, p.nprof_i, p.nprof_z,

/* The u-band AperFlux */
up0.profMean as uAperFlux0, up1.profMean as uAperFlux1, 
up2.profMean as uAperFlux2, up3.profMean as uAperFlux3, 
up4.profMean as uAperFlux4, up5.profMean as uAperFlux5, 
up6.profMean as uAperFlux6, up7.profMean as uAperFlux7, 

/* The g-band AperFlux */
gp0.profMean as gAperFlux0, gp1.profMean as gAperFlux1, 
gp2.profMean as gAperFlux2, gp3.profMean as gAperFlux3, 
gp4.profMean as gAperFlux4, gp5.profMean as gAperFlux5, 
gp6.profMean as gAperFlux6, gp7.profMean as gAperFlux7,

rp0.profMean as rAperFlux0, rp1.profMean as rAperFlux1, 
rp2.profMean as rAperFlux2, rp3.profMean as rAperFlux3, 
rp4.profMean as rAperFlux4, rp5.profMean as rAperFlux5, 
rp6.profMean as rAperFlux6, rp7.profMean as rAperFlux7,

ip0.profMean as iAperFlux0, ip1.profMean as iAperFlux1, 
ip2.profMean as iAperFlux2, ip3.profMean as iAperFlux3, 
ip4.profMean as iAperFlux4, ip5.profMean as iAperFlux5, 
ip6.profMean as iAperFlux6, ip7.profMean as iAperFlux7,

zp0.profMean as zAperFlux0, zp1.profMean as zAperFlux1, 
zp2.profMean as zAperFlux2, zp3.profMean as zAperFlux3, 
zp4.profMean as zAperFlux4, zp5.profMean as zAperFlux5, 
zp6.profMean as zAperFlux6, zp7.profMean as zAperFlux7

/* mydb.sdssmpa_rowind contains the SDSS-MPA rowindex and specobjid for all galaxies */
FROM specobj as s, photoobjall as p, mydb.sdssmpa_rowind as m, 
PhotoProfile as up0, PhotoProfile as gp0, PhotoProfile as rp0, PhotoProfile as ip0,
PhotoProfile as zp0,
PhotoProfile as up1, PhotoProfile as gp1, PhotoProfile as rp1, PhotoProfile as ip1,
PhotoProfile as zp1,
PhotoProfile as up2, PhotoProfile as gp2, PhotoProfile as rp2, PhotoProfile as ip2,
PhotoProfile as zp2,
PhotoProfile as up3, PhotoProfile as gp3, PhotoProfile as rp3, PhotoProfile as ip3,
PhotoProfile as zp3,
PhotoProfile as up4, PhotoProfile as gp4, PhotoProfile as rp4, PhotoProfile as ip4,
PhotoProfile as zp4,
PhotoProfile as up5, PhotoProfile as gp5, PhotoProfile as rp5, PhotoProfile as ip5,
PhotoProfile as zp5,
PhotoProfile as up6, PhotoProfile as gp6, PhotoProfile as rp6, PhotoProfile as ip6,
PhotoProfile as zp6,
PhotoProfile as up7, PhotoProfile as gp7, PhotoProfile as rp7, PhotoProfile as ip7,
PhotoProfile as zp7
 

/* Join Specobj, PhotoobjAll, SDSSMPA_rowind and select only
spectroscopic galaxies */
WHERE s.specobjid=p.specobjid AND s.specobjid=m.specobjid AND s.specclass=2 AND 


\end{verbatim}
\end{code*}

\begin{code*}
\begin{verbatim}


/* Join u-band PhotoProfiles */
s.bestobjid = up0.objid AND up0.band = 0 AND up0.bin = 0 AND
s.bestobjid = up1.objid AND up1.band = 0 AND up1.bin = 1 AND 
s.bestobjid = up2.objid AND up2.band = 0 AND up2.bin = 2 AND 
s.bestobjid = up3.objid AND up3.band = 0 AND up3.bin = 3 AND 
s.bestobjid = up4.objid AND up4.band = 0 AND up4.bin = 4 AND
s.bestobjid = up5.objid AND up5.band = 0 AND up5.bin = 5 AND
s.bestobjid = up6.objid AND up6.band = 0 AND up6.bin = 6 AND
s.bestobjid = up7.objid AND up7.band = 0 AND up7.bin = 7 AND

/* Join g-band PhotoProfiles */
s.bestobjid = gp0.objid AND gp0.band = 1 AND gp0.bin = 0 AND
s.bestobjid = gp1.objid AND gp1.band = 1 AND gp1.bin = 1 AND 
s.bestobjid = gp2.objid AND gp2.band = 1 AND gp2.bin = 2 AND 
s.bestobjid = gp3.objid AND gp3.band = 1 AND gp3.bin = 3 AND 
s.bestobjid = gp4.objid AND gp4.band = 1 AND gp4.bin = 4 AND
s.bestobjid = gp5.objid AND gp5.band = 1 AND gp5.bin = 5 AND
s.bestobjid = gp6.objid AND gp6.band = 1 AND gp6.bin = 6 AND
s.bestobjid = gp7.objid AND gp7.band = 1 AND gp7.bin = 7 AND

/* Join r-band PhotoProfiles */
s.bestobjid = rp0.objid AND rp0.band = 2 AND rp0.bin = 0 AND
s.bestobjid = rp1.objid AND rp1.band = 2 AND rp1.bin = 1 AND 
s.bestobjid = rp2.objid AND rp2.band = 2 AND rp2.bin = 2 AND 
s.bestobjid = rp3.objid AND rp3.band = 2 AND rp3.bin = 3 AND 
s.bestobjid = rp4.objid AND rp4.band = 2 AND rp4.bin = 4 AND
s.bestobjid = rp5.objid AND rp5.band = 2 AND rp5.bin = 5 AND
s.bestobjid = rp6.objid AND rp6.band = 2 AND rp6.bin = 6 AND
s.bestobjid = rp7.objid AND rp7.band = 2 AND rp7.bin = 7 AND

/* Join i-band PhotoProfiles */
s.bestobjid = ip0.objid AND ip0.band = 3 AND ip0.bin = 0 AND
s.bestobjid = ip1.objid AND ip1.band = 3 AND ip1.bin = 1 AND 
s.bestobjid = ip2.objid AND ip2.band = 3 AND ip2.bin = 2 AND 
s.bestobjid = ip3.objid AND ip3.band = 3 AND ip3.bin = 3 AND 
s.bestobjid = ip4.objid AND ip4.band = 3 AND ip4.bin = 4 AND
s.bestobjid = ip5.objid AND ip5.band = 3 AND ip5.bin = 5 AND
s.bestobjid = ip6.objid AND ip6.band = 3 AND ip6.bin = 6 AND
s.bestobjid = ip7.objid AND ip7.band = 3 AND ip7.bin = 7 AND

/* Join z-band PhotoProfiles */
s.bestobjid = zp0.objid AND zp0.band = 4 AND zp0.bin = 0 AND
s.bestobjid = zp1.objid AND zp1.band = 4 AND zp1.bin = 1 AND 
s.bestobjid = zp2.objid AND zp2.band = 4 AND zp2.bin = 2 AND 
s.bestobjid = zp3.objid AND zp3.band = 4 AND zp3.bin = 3 AND 
s.bestobjid = zp4.objid AND zp4.band = 4 AND zp4.bin = 4 AND
s.bestobjid = zp5.objid AND zp5.band = 4 AND zp5.bin = 5 AND
s.bestobjid = zp6.objid AND zp6.band = 4 AND zp6.bin = 6 AND
s.bestobjid = zp7.objid AND zp7.band = 4 AND zp7.bin = 7


\end{verbatim}
\end{code*}

\clearpage


\begin{code*}
{\bf /*To obtain parameters for UKIDSS sources which are spectroscopic galaxies
in the SDSS. */}
\begin{verbatim}
SELECT  ss.specobjid, ls.sourceid, x.distancemins, 

/* Petrosian magnitudes */
ls.yPetroMag, ls.j_1PetroMag, ls.hPetroMag, ls.kPetroMag, 

/* dust attenuation */
ls.aY, ls.aH, ls.aJ, ls.aK,

/* Petrosian radii */
yd.PetroRad as yPetroRad, jd.PetroRad as j_1PetroRad, hd.PetroRad as hPetroRad, 
kd.PetroRad as kPetroRad, 

/* UKIDSS Aper mags */
yd.Aperflux1 as yAperFlux1, jd.AperFlux1 as j_1AperFlux1, hd.AperFlux1 as hAperFlux1, 
kd.AperFlux1 as kAperFlux1,
yd.Aperflux2 as yAperFlux2, jd.AperFlux2 as j_1AperFlux2, hd.AperFlux2 as hAperFlux2, 
kd.AperFlux2 as kAperFlux2,
yd.Aperflux3 as yAperFlux3, jd.AperFlux3 as j_1AperFlux3, hd.AperFlux3 as hAperFlux3, 
kd.AperFlux3 as kAperFlux3,
yd.Aperflux4 as yAperFlux4, jd.AperFlux4 as j_1AperFlux4, hd.AperFlux4 as hAperFlux4, 
kd.AperFlux4 as kAperFlux4,
yd.Aperflux5 as yAperFlux5, jd.AperFlux5 as j_1AperFlux5, hd.AperFlux5 as hAperFlux5, 
kd.AperFlux5 as kAperFlux5,
yd.Aperflux6 as yAperFlux6, jd.AperFlux6 as j_1AperFlux6, hd.AperFlux6 as hAperFlux6, 
kd.AperFlux6 as kAperFlux6,
yd.Aperflux7 as yAperFlux7, jd.AperFlux7 as j_1AperFlux7, hd.AperFlux7 as hAperFlux7, 
kd.AperFlux7 as kAperFlux7,
yd.Aperflux8 as yAperFlux8, jd.AperFlux8 as j_1AperFlux8, hd.AperFlux8 as hAperFlux8, 
kd.AperFlux8 as kAperFlux8,
yd.Aperflux9 as yAperFlux9, jd.AperFlux9 as j_1AperFlux9, hd.AperFlux9 as hAperFlux9, 
kd.AperFlux9 as kAperFlux9,
yd.Aperflux10 as yAperFlux10, jd.AperFlux10 as j_1AperFlux10, hd.AperFlux10 as hAperFlux10, 
kd.AperFlux10 as kAperFlux10,
yd.Aperflux11 as yAperFlux11, jd.AperFlux11 as j_1AperFlux11, hd.AperFlux11 as hAperFlux11, 
kd.AperFlux11 as kAperFlux11,
yd.Aperflux12 as yAperFlux12, jd.AperFlux12 as j_1AperFlux12, hd.AperFlux12 as hAperFlux12, 
kd.AperFlux12 as kAperFlux12,

/* J band exposure time */
mf.expTime

FROM lasYJHKSource AS ls,  bestdr7..specobj as ss, lasSourceXDR7PhotoObj as x, 
lasYJHKMergeLog AS ml, lasDetection as jd, lasdetection as hd, lasdetection as yd, 
lasdetection as kd, multiframe as mf

WHERE x.masterobjid=ls.sourceid AND ss.bestobjid=x.slaveobjid AND 
ls.framesetID = ml.framesetID AND ml.j_1mfID = mf.multiframeID AND

/* Join merge log to detection for the J frame: */
ml.j_1mfID = jd.multiframeID AND ml.j_1eNum = jd.extNum AND
/* Join source to detection to look up the detection required: */
ls.j_1SeqNum = jd.seqNum AND 

/* Join merge log to detection for the Y frame: */
ml.ymfID = yd.multiframeID AND ml.yeNum = yd.extNum AND
/* Join source to detection to look up the detection required: */
ls.ySeqNum = yd.seqNum AND 
\end{verbatim}
\end{code*}

\begin{code*}
\begin{verbatim}

/* Join merge log to detection for the H frame: */
ml.hmfID = hd.multiframeID AND ml.heNum = hd.extNum AND
/* Join source to detection to look up the detection required: */
ls.hSeqNum = hd.seqNum AND 

/* Join merge log to detection for the K frame: */
ml.kmfID = kd.multiframeID AND ml.keNum = kd.extNum AND
/* Join source to detection to look up the detection required: */
ls.kSeqNum = kd.seqNum AND 

/* remove blended objects */
ls.yppErrBits&0x00000010 = 0 AND ls.j_1ppErrBits&0x00000010 = 0 AND 
ls.hppErrBits&0x00000010 = 0 AND ls.kppErrBits&0x00000010 = 0 AND

/* now get spectroscopic galaxies and select the nearest match */
ss.specclass=2 AND distanceMins<0.033333 AND 
distanceMins IN ( SELECT MIN(distanceMins) FROM lasSourceXDR7PhotoObj 
WHERE masterObjID=x.masterObjID AND sdssPrimary=1)
\end{verbatim}
\end{code*}

\clearpage

\begin{code*}
{\bf /*To obtain parameters for GALEX sources which are spectroscopic galaxies
in the SDSS. */}
\begin{verbatim}

/* Basic parameters */
SELECT ss.bestobjid, ss.specobjid, gg.objid, gg.distance, gg.reversemultiplematchcount,

/* GALEX Fluxes */  
ga.nuv_flux, ga.nuv_fluxerr,ga.fuv_flux, ga.fuv_fluxerr, ga.e_bv

/* myDB.dr7SFgal contains an uploaded list of all the specobjids we want to match */
FROM myDB.dr7SFgal as ss, galexgr4plus5..xsdssdr7 as gg, galexgr4plus5..photoobj as ga

WHERE ss.bestobjid=gg.SDSSobjid and gg.objid=ga.objid and gg.reversedistancerank=1

\end{verbatim}
\end{code*}

